Priority-based Parameter Propagation for Distributed DNN Training

Data parallel training is widely used for scaling distributed deep neural network (DNN) training. However, the performance benefits are often limited by the communication-heavy parameter synchronization step. In this paper, we take advantage of the domain specific knowledge of DNN training and overlap parameter synchronization with computation in order to improve the training performance. We make two key observations: (1) the optimal data representation granularity for the communication may differ from that used by the underlying DNN model implementation and (2) different parameters can afford different synchronization delays. Based on these observations, we propose a new synchronization mechanism called Priority-based Parameter Propagation (P3). P3 synchronizes parameters at a finer granularity and schedules data transmission in such a way that the training process incurs minimal communication delay. We show that P3 can improve the training throughput of ResNet-50, Sockeye and VGG-19 by as much as 25%, 38% and 66% respectively on clusters with realistic network bandwidth

==> Makefile <==
PAPER = sysml
TEX = $(wildcard *.tex sections/*.tex figNodes/*.tex)
BIB = sysml.bib
FIGS = $(wildcard plots/*.pdf plots/*.png)

.PHONY: all clean

$(PAPER).pdf: $(TEX)  $(BIB) $(FIGS) 
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi *.gz \
	$(PAPER).pdf


==> future.tex <==
\section{Future Work}

==> motivation.tex <==
\section{Motivation and Analysis}
\begin{figure}[h]
	\centering
	\includegraphics[width=60mm]{plots/nw-tp}
	\caption{Network vs Throughput of ResNet-50 on MXNet}
	\label{fig:nw-tp}
\end{figure}
\begin{figure}[h]
	\centering
	\subfigure[MXNet]{
		\label{fig:mxnet-nw}
		\includegraphics[width=60mm]{"plots/nw-util-mxnet"}
	}
	\subfigure[TensorFlow]{
		\label{fig:tf-nw}
		\includegraphics[width=60mm]{plots/nw-util-tf}
	}
	\label{fig:nw-util}
	\caption{Network utilization of ResNet-50 at 4Gbps bandwidth}
\end{figure}

For this work, we started by examining distributed training of ResNet-50 over TensorFlow and MXNet on a 4 node cluster. We measured the training throughput and the network utilization of the worker machines while artificially limiting the network interface peak transmission rate starting from 10Gbps down to 1Gbps. As shown in Figure \ref{fig:nw-tp}, the throughput start to drop from 5Gbps onwards and at 4Gbps it drops by $25\%$ of the original throughput. However, at the same time the network is observed to be underutilized. Figure \ref{fig:nw-util} shows the inbound and outbound traffic from one of the worker machines during training. These regular peaks and following idle time in the traffic pattern suggests that even though the network bandwidth is not sufficient enough, the training process fails to fully utilize the available network bandwidth.

\begin{figure*}[h]
	\centering
	\subfigure[ResNet-50]{
		\label{fig:dist-resnet}
		\includegraphics[width=40mm]{plots/skew-resnet50}
	}
	\subfigure[InceptionV3]{
		\label{fig:dist-incep}
		\includegraphics[width=40mm]{plots/skew-incep}
	}
	\subfigure[VGG-19]{
		\label{fig:dist-vgg}
		\includegraphics[width=40mm]{plots/skew-vgg}
	}
	\subfigure[Sockeye]{
		\label{fig:dist-sockeye}
		\includegraphics[width=40mm]{plots/skew-sockeye}
	}
	\caption{Parameter distribution}
	\label{fig:dist}
\end{figure*}
Further analysis revealed that these gaps in the network utilization graphs occur during the forward propagation. Since the frameworks aggressively send the gradients without accounting for when they are going to be consumed, on a bandwidth constrained network, later layers can induce queuing delay on to the initial layers. This prevents the communication from overlapping with the subsequent forward propagation.
\begin{figure}[h]
	\centering
	\subfigure[Aggressive synchronization]{
		\label{fig:delay-bad}
		\includegraphics[width=60mm]{"plots/delay-bad"}
	}
	\subfigure[Priority based synchronization]{
		\label{fig:delay-fix}
		\includegraphics[width=60mm]{plots/delay-fix}
	}
	\label{fig:delay}
	\caption{Parameter synchronization}
\end{figure}

For example, in Figure \ref{fig:delay-bad}, the 3 layered DNN takes 1 time step to compute gradients of a layer and 2 time steps for synchronizing parameters of that layer. With aggressive parameter synchronization the total delay incurred for the next iteration is twice that of the time needed to synchronize the first layer parameters. This effect becomes more dominant when the communication time required for individual layers vary due the presence dense layers in the DNN. Under limited bandwidth, the heavy final layers of ResNet-50 induces additional queuing delay on to the following layers.

As shown in figure \ref{fig:dist} this skewed parameter distribution is a general trend in the image classification models where the size of the layer increases considerably from initial layers to final ones. Since the gradients of the final layers are computed at the beginning of the backward propagation and consumed at the end of the next forward propagation, it gives more room for the heavy final layers to overlap parameter update with the computation compared to the lighter initial layers. In \name, we are taking advantage of this unique characteristics of DNN models.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\textwidth]{"plots/nw-vgg"}
	\caption{Network utilization of VGG-19}
	\label{fig:nw-vgg}
\end{figure}
Secondly, we examined distributing larger DNNs like VGG-19 and observed the traffic. Network utilization graphs of VGG-19 is highly irregular as shown in figure \ref{fig:nw-vgg}. On top of that, the inbound and outbound traffic are not completely overlapped. The reason behind this is because VGG-19 contains a single fully connected layer which consist of $71.5\%$ of the parameters in the whole network (Figure \ref{fig:dist-vgg}). Since the synchronization of this layer cannot be overlapped with other layers, they end up underutilizing both its computing resources as well as bidirectional bandwidth. As shown in Figure \ref{fig:pipe-bad}, the second heavy layer takes thrice as much time to synchronize than the first and third. Because of this imbalance synchronization of second layer becomes the critical path and fail to overlap well with the other 2 layers. This causes under utilization of compute resources and bidirectional bandwidth.

\begin{figure}[h]
	\centering
	\subfigure[At layer-wise granularity]{
		\label{fig:pipe-bad}
		\includegraphics[width=60mm]{"plots/pipe-bad"}
	}
	\subfigure[At finer granularity]{
		\label{fig:pipe-fix}
		\includegraphics[width=60mm]{plots/pipe-fix}
	}
	\label{fig:pipe}
	\caption{Pipelining parameter synchronization}
\end{figure}

From the above observations we draw 2 conclusions:
\begin{itemize}
	\item Application domain-specific knowledge of DNNs can be utilized to schedule communication not only based on when data is generated but also on when they are going to be consumed.
	\item The optimal granularity required for parameter synchronization may differ from the one used for data representation by the underlying model implementation.
\end{itemize}
